Algorithms for Recursive Block Matrices

We study certain linear algebra algorithms for recursive block matrices. This representation has useful practical and theoretical properties. We summarize some previous results for block matrix inversion and present some results on triangular decomposition of block matrices. The case of inverting matrices over a ring that is neither formally real nor formally complex was inspired by Gonzalez-Vega et al.

==> IfExistsUseBBL.tex <==
% This file must not be empty, otherwise arXiv removes it.
